Quantifying the Carbon Reduction of DAG Workloads: A Job Shop Scheduling Perspective

Carbon-aware schedulers aim to reduce the operational carbon footprint of data centers by running flexible workloads during periods of low carbon intensity. Most schedulers treat workloads as single monolithic tasks, ignoring that many jobs, like video encoding or offline inference, consist of smaller tasks with specific dependencies and resource needs; however, knowledge of this structure enables opportunities for greater carbon efficiency. We quantify the maximum benefit of a dependency-aware approach for batch workloads. We model the problem as a flexible job-shop scheduling variant and use an offline solver to compute upper bounds on carbon and energy savings. Results show up to $25\%$ lower carbon emissions on average without increasing the optimal makespan (total job completion time) compared to a makespan-only baseline. Although in heterogeneous server setup, these schedules may use more energy than energy-optimal ones. Our results also show that allowing twice the optimal makespan nearly doubles the carbon savings, underscoring the tension between carbon, energy, and makespan. We also highlight key factors such as job structure and server count influence the achievable carbon reductions.

==> 1-introduction.tex <==



In recent years, increasing demand for computing and growth in new data center projects have prompted concerns about the electricity needs and resulting operational carbon footprint of Information and Communications Technology~\cite{GoldmanSachs:25, Shehabi2024:USDCReport}.  Data center operators have previously addressed these concerns by optimizing the \textit{energy efficiency} of their operations~\cite{Barroso_warehouse}, but these improvements are quickly approaching fundamental limits with the advent of hyperscale data centers~\cite{Bashir:23}.  
Thus, future growth in demand is expected to increase energy usage significantly~\cite{Shehabi2024:USDCReport} -- since the favored choices for new power generation to support data centers continue to be fossil-based resources such as natural gas turbines~\cite{NYT:25GasTurbines, skidmore2025:Stargate}, this projected growth is expected to correlate with increases in carbon emissions.

% Combined with a desire for consistent (i.e., \textit{not} intermittent) power,  as  \walid{I have a small concern on saying that the solution is non intermittent and then talking about how we use it :D}

% Future growth in demand and desires for consistent power are now projected to incre

% Thus, future growth in demand is now expected to increase energy usage and thus increase carbon emissions as a result. 

% \walid{So, what? e.g., we can say that despite the challenges in meeting the huge energy increase, these increases is often correlated with increases in carbon emissions as most grids are powered by fossil... }

% Furthermore, societal trends in electrification (e.g., in residential heating, transportation) promise to exacerbate strain on grids worldwide~\cite{Blonsky:19}. \walid{not sure how electrification is relevant}

% \adaml{classical introduction about carbon emissions in the data center compute}

To address concerns about carbon footprint,
data center operators have sometimes turned to \textit{supply-side} optimizations, e.g., by purchasing renewable power or co-locating data centers with wind and solar farms~\cite{Acun:23, GoogleRenewableEnergy:18, Calma:24}.
% however, such approaches can be costly\walid{not always e.g., if you matched the energy somewhere else}
Researchers have also proposed \textit{demand-side} techniques in recent years to reduce the operational carbon of batch workloads using temporal or spatial 
% shifting~\cite{wait-awhile, sukprasert:2023:quantifying, hanafy:2023:carbonscaler, Zheng:20, lin2023adapting, wu2025:CarbonEdge, Gsteiger:24}.  
shifting~\cite{wait-awhile, sukprasert:2023:quantifying, hanafy:2023:carbonscaler, Zheng:20, lin2023adapting, Gsteiger:24}.  
These works rely on visibility into the grid's \textit{carbon intensity} (i.e., amount of carbon emitted per unit of energy used) and flexible applications that can modulate in response to variations on the grid.
Existing works run the gamut from theoretical models that consider single jobs with deadlines
% ~\cite{Lechowicz:23, Lechowicz:24, bostandoost:2024:lacs} 
~\cite{Lechowicz:23} 
to experimental techniques that provision the resources available for multiple jobs in response to carbon intensity~\cite{radovanovic2022carbon, souza:2023:ecovisor, Acun:23, Chadha:23, Gsteiger:24, perotin2023risk}. 
% \walid{Dial down our citations for this version, prashant is in 25\% of the refs :D -- may be keep CS, DTPR, Eco visor, tammy and war of efficiency only, we can add more in the camera ready.}

% \adaml{two views: supply side vs. demand side, techniques in each -- demand response or demand shifting}

However, despite the variety of settings that have already been explored, these works mostly cast each workload as a \textit{single monolithic task} in the sense that each job has a single resource requirement (resp. scaling profile) and a single length.  In reality, many batch compute workloads in the data center that are candidates for carbon-aware shifting can be decomposed into distinct tasks with dependencies (e.g., the input of one task is the output of another). Examples of background jobs with this structure include video encoding/transcoding, serverless processing~\cite{Kounev2023:Serverless}, storage management~\cite{Rao:25}, offline inference, and others~\cite{Alibaba:19, wei2022status}.
Similarly, the data center resources that tasks can be scheduled on are often diverse (e.g., CPU-only vs. GPU machines or different hardware generations), and may exhibit different energy and performance profiles for each job. For instance, in \autoref{fig:motivation-dag}, we discuss a motivating example to show how a simple dependency structure between four tasks can force a divergence between the attempted and realized schedules of a \textit{dependency-unaware} scheduler, resulting in an unplanned ``spillover'' into a high-carbon period.

While recent work has begun to explore dependency-aware and carbon-aware workload scheduling~\cite{Gsteiger:24}, their solution is based on heuristics. These operators need to know whether improving their approaches is worth it or not. The first step to answer this question is to quantify how much the upper bound of this improvement could be when all the information,e.g., the job arrivals, task dependencies, and their energy utilization profile on each server, is known beforehand.
We consider scheduling batch workloads since they constitute a good portion of datacenter workloads.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/motivation2.png} \vspace{-1em}
    \caption{
    Given four tasks with dependencies, a carbon-aware but dependency-\textit{unaware} scheduler attempts to run all tasks (in parallel) at the low-carbon period.  However, due to dependencies, the only task that can run at that time is task 1, pushing other tasks to a high-carbon period.  In contrast, a dependency-aware scheduler sacrifices the carbon footprint of task $1$ to gain more on other tasks (i.e., tasks 2-4).
    }
    \label{fig:motivation-dag} \vspace{-1em}
\end{figure}

To answer this question, we borrow the concept of the job shop scheduling domain in operations research. In operations research, the flow shop, job shop, and flexible job shop scheduling problems have been studied for decades~\cite{Emmons:12, Manne:60, Xiong:22, Dauzere:24, Graham:66}.  
In computer science, scheduling for precedence-constrained tasks has been approached through online algorithms and heuristics that primarily seek to minimize makespan (i.e., total completion time), for problem domains where tasks with dependencies are common, such as epigenetics scientific workloads and data processing~\cite{coleman:25:pisaadversarialapproachcomparing}.
In this work, we study a variant of the flexible job shop scheduling problem (FJSP) with an objective of energy usage or operational carbon emissions, subject to a specified constraint on the makespan. 
We compare the results achievable for this formulation against the standard FJSP with a makespan objective, characterizing the degree to which there is a trade-off (i.e., conflict) between the studied objectives.
We construct instances of FJSP where each job is composed of a dependency graph and tasks that resemble real-world workloads from Alibaba cluster traces~\cite{Alibaba:18}.
We combine these instances with carbon intensity traces from Electricity Maps~\cite{electricity-map}, and use an offline constraint optimization solver~\cite{ortools} to explore the feasible space of schedules that trade-off between carbon footprint, energy usage, and total makespan.

\noindent \textbf{Contributions: } We quantify potential improvements and highlight the challenges:
\begin{enumerate}[leftmargin=*]
\item In our experiments, we show that a carbon-aware solver with fine-grained information about inter-task dependencies can achieve carbon reductions of up to 25\% without increasing overall makespan.
\item We find a \textit{tension} between optimizing for carbon emissions and optimizing for energy usage in the FJSP -- these objectives are sometimes complementary, but sometimes in conflict.
\item Our analysis emphasizes the complexity of solving the FJSP and highlights challenges for scheduling such workloads in realistic data center settings.  We sketch a potential roadmap of approaches to address these and realize the carbon benefits of dependency-awareness.
\end{enumerate}

% However, despite the variety of settings that have already been explored, these works mostly cast each workload as a \textit{black-box} in the sense that each job has a single resource requirement (resp. scaling profile) and a single length.  In reality, many batch compute workloads in the data center that are candidates for carbon-aware shifting can be decomposed into distinct tasks with dependencies (e.g., the input of one task is the output of another).  Examples of background jobs with this structure include video encoding/transcoding, serverless processing~\cite{Kounev2023:Serverless}, storage management~\cite{Rao:25}, offline inference, and others~\cite{Alibaba:19, wei2022status}.
% Furthermore, the constituent tasks of each workload often exhibit different energy and resource requirements and/or scaling profiles, resulting in different operational carbon footprints.  
% Similarly, the data center resources that tasks can be scheduled on are often diverse (e.g., CPU-only vs. GPU machines or different hardware generations), and may exhibit different energy and performance profiles for each job.  While existing work in carbon-aware shifting usually ignores these \textit{fine-grained details} of inter-task dependencies and resource heterogeneity for each job, they must be considered to be optimally carbon-aware.  
% For instance, in \autoref{fig:motivation-dag}, we discuss a motivating example to show how a simple dependency structure between four tasks can force a divergence between the attempted and realized schedules of a \textit{dependency-unaware} scheduler, resulting in an unplanned ``spillover'' into a high-carbon period.

% \rev{While recent work has begun to explore dependency-aware scheduling for carbon-aware serverless workflows~\cite{Gsteiger:24}, the rich internal structure of traditional batch workloads (e.g., video encoding, offline inference, storage management~\cite{Rao:25}) remains a largely untapped source of flexibility for carbon optimization. Many of these workloads can be decomposed into distinct tasks with dependencies and heterogeneous resource requirements. Ignoring these fine-grained details can lead to suboptimal schedules; for instance, a dependency-unaware scheduler might attempt to run all tasks in a low-carbon period, only to find that dependencies force tasks into a high-carbon "spillover" period (\autoref{fig:motivation-dag}).}

% \rb{we can replace blue with red}


% Inter-task dependencies have been extensively considered from a performance perspective in other domains. In operations research, the flow shop, job shop, and flexible job shop scheduling problems have been studied for decades~\cite{Emmons:12, Manne:60, Xiong:22, Dauzere:24, Graham:66}.  
% In computer science, scheduling for precedence-constrained tasks has been approached through online algorithms and heuristics that primarily seek to minimize makespan (i.e., total completion time), for problem domains where tasks with dependencies are common, such as epigenetics scientific workloads and data processing~\cite{coleman:25:pisaadversarialapproachcomparing}.

% In this work, we study a variant of the flexible job shop scheduling problem (FJSP) with an objective of energy usage or \rb{operational} carbon emissions, subject to a specified constraint on the makespan. 

% \rb{Maybe we need to add a few sentences on why we did not consider embodied carbon footprint.}
% \AL{I think this would be good since reviewers will ask either way (unfortunately)}

% We compare the results achievable for this formulation against the standard FJSP with a makespan objective, characterizing the degree to which there is a trade-off (i.e., conflict) between the studied objectives.
% We construct instances of FJSP where each job is composed of a dependency graph and tasks that resemble real-world workloads from Alibaba cluster traces~\cite{Alibaba:18}.

% We combine these instances with carbon intensity traces from Electricity Maps~\cite{electricity-map}, and use an offline constraint optimization solver~\cite{ortools} to explore the feasible space of schedules that trade-off between carbon footprint, energy usage, and total makespan.


% \noindent \textbf{Contributions: } We highlight several opportunities and challenges:
% \begin{enumerate}[leftmargin=*]
% \item In our experiments, we show that a carbon-aware solver with fine-grained information about inter-task dependencies can achieve carbon reductions of up to 25\% without increasing overall makespan.  
% \item We find a \textit{tension} between optimizing for carbon emissions and optimizing for energy usage in the FJSP -- these objectives are sometimes complementary, but sometimes in conflict.
% \item Our analysis emphasizes the complexity of solving the FJSP and highlights challenges for scheduling such workloads in realistic data center settings.  We sketch a potential roadmap of approaches to address these and realize the carbon benefits of dependency-awareness.
% \end{enumerate}


% In doing so, we illuminate paths for future research directions into practical online carbon-aware schedulers that could be applied to make fine-grained scheduling decisions in carbon-aware data centers.  

% {\color{blue} Our findings identify both opportunities and challenges -- for instance, our preliminary results show that a carbon- and dependency-aware schedule can achieve carbon reductions of up to \rev{30\%} without increasing makespan (e.g., by shifting idle periods), at the expense of requiring fine-grained information about the individual tasks that constitute the workloads in the system.}

% \walid{Are we presenting contributions or just this?}

% \adaml{eventually I think contributions -- I will revise the section in blue}

% \adaml{key takeaways so far:}

% \adaml{carbon savings without makespan}
% \adaml{carbon and energy tension}
% \adaml{complexity of the problem -- online schedulers needed}
% \adaml{I took an initial pass over these contributions above}


% {\color{blue}
% \adaml{suggested outline}

% \begin{itemize}
%     \item several techniques have been proposed to reduce the operational carbon of computing through temporal or spatial shifting
%     \item However, most of these works view jobs as a black-box...
%     \item in reality, many compute workloads can be decomposed into stages, input of one stage is the output of another, and this is also true for background tasks / non-interactive jobs in the data center that would be good candidates for carbon-aware load shifting
%     \item example: video encoding/transcoding (e.g., YouTube or Zoom servers)
%     \begin{itemize}
%         \item discrete steps in this pipeline: e.g., multi-bitrate encoding, codec optimization, segmentation
%     \end{itemize}
%     \item example: batch inference (MSR)
%     \begin{itemize}
%         \item  
%     \end{itemize}
%     \item Furthermore, the stages of a job may exhibit different energy \& resource requirements, and thus different carbon footprints as a result.
%     \item while dependencies of this form have not yet been considered in the context of carbon-aware scheduling, they have been extensively considered in other literature...
%     \item In this work, we study the flexible job shop scheduling problem (FJSP) under the conflicting objectives of makespan and carbon emissions.
%     \item we construct instances of FJSP, combine them with carbon traces from electricity map, and use an offline constraint optimization solver to explore the feasible space of schedules that trade-off between carbon and makespan.
%     \item our contributions illuminate paths for future research directions in practical online carbon-aware schedulers.  
%     \item In particular, (opportunities) and (challenges)
% \end{itemize}

% }

==> 4-discussion-v2.tex <==
% \noindent{\textbf{What we learn.}} We find FJSP instances where a dependency-aware, carbon-aware schedule cuts \textit{operational} emissions with no makespan increase ($S=1$). This happens when the makespan-optimal (carbon-agnostic) schedule leaves \textit{idle gaps} that we can shift into low-carbon windows. As those gaps shrink, e.g., due to more operations per job, savings drop (\autoref{tab:num-ops}). These results are upper bounds from an offline, perfect-foresight analysis and help operators decide whether improving their current algorithm or heuristic is worth the effort given the upper-bound gains.

% \noindent{\textbf{Carbon vs.\ energy.}} Carbon-optimal schedules do not always minimize total energy. We see cases where energy falls while carbon rises, because the schedule stretches work into high-carbon periods. This trade-off should shape the scheduling policy design.

% \noindent{\textbf{Why we need online algorithms.}} As $S$ grows, the offline search space explodes; some instances hit time limits and yield weaker schedules. Real schedulers also lack oracle inputs (exact arrivals, task times, future carbon). We therefore need \textbf{online} methods that (i) run fast at scale, (ii) work with predictions or partial information, and (iii) come with \textit{theoretical guarantees}—e.g., competitive ratios, approximation bounds, or regret guarantees under forecast error. The goal is simple: keep makespan near-optimal while capturing a \textit{provable} slice of the carbon savings our offline study reveals.


% \noindent{\textbf{What we did not model.}} A server's idle power~\cite{Lefurgy:07}, energy proportionality~\cite{Barroso_warehouse}, and task parallelization limits (i.e., if a task is parallelizable)~\cite{fernandez2025hardwarescalingtrendsdiminishing}. These factors can shift where and how much savings appear.

% In short, our offline study maps the headroom. The next step is online, prediction-aware schedulers that run fast, need no oracle, and carry clear guarantees on carbon and performance.
%-------------------------------------------------------
% \rb{make it two sections: lessons learned: tradeoffs, parameters effect: ops, servers, regions, limitations: emobided, full info}
% \rb{In addition in war of efficicies, we learn that heterogenity can also rise the tension btw energy vs. carbon. prior works(cite) should also consider this setup when optimizing for carbon alongside energy.}
% \rb{mention balancing the tradeoff with coeff}

\rb {mention reordering tasks to save carbon that can incentivize heuristic design}

\rb {we highliught following key insights to better help operators design online heurisitics}

\rb {1) we highlighted the potential, the tradeoffs: savings without sacrificing makespan (lower utilization), maximizing savings -> sacrificing makespan (diminishing returns), we also highlightted in hetreogeneous settings tradeoff between carbon vs. energy (GPU clusters)}


\noindent{\textbf{Key insights.}} Prior work~\cite{Hanafy:23:War} showed that workload scheduling mechanisms often face a trade-off between carbon efficiency, energy efficiency, and performance in homogeneous clusters. Our work reveals that server heterogeneity intensifies this conflict. For instance, running a workload on a faster, less energy-efficient server during a high-carbon period might save energy but will ultimately increase carbon emissions, while using a faster, less efficient server on low-carbon periods may lower emissions but waste energy. 
% We found that a carbon-aware schedule, when given $2\times$ the optimal makespan flexibility, cut carbon emissions by half but $7\%$ more energy consumption than the energy-aware schedule.
% \walid{disconnected -- may be talk about how make span affect this trade-off}
Our offline solver provides \textit{upper bounds on achievable savings}. With $2\times$ the optimal makespan flexibility, a carbon-aware schedule emits $20\%$ less carbon but uses $7\%$ more energy than the energy-aware schedule. This result quantifies the limits of what an idealized scheduler could achieve, and helps operators judge whether refining their existing policies is worth the effort. 

This trade-off matters for works on heterogeneous environments, such as energy-efficient GPU clusters~\cite{enos2010quantifying, ma2012greengpu}: cluster heterogeneity must be considered if carbon efficiency is also a goal alongside energy efficiency. Operators can tune how much they value carbon versus energy by assigning explicit weights to each.  
We also quantify the carbon–makespan trade-off. Longer makespans create more chances to exploit low-carbon windows. In our runs, doubling the makespan nearly doubled the savings. 

% Finally, we identify parameters that shape carbon savings (compared to the makespan-minimizer solver). Increasing tasks per job from 3 to 5 increased server utilization by an average of 20\%, which reduced carbon savings by 10\%. Increasing servers from 2 to 5 halved server utilization on average and produced up to $20\times$ higher carbon savings. 

Finally, we identify parameters that shape carbon savings relative to the makespan-only baseline. Increasing tasks per job from 3 to 5 raised server utilization by 20\% on average and reduced savings by 10\%. In contrast, increasing servers from 2 to 5 halved utilization and boosted savings by up to $20\times$.


% \noindent{\textbf{Limitations.}} The main challenge is the complexity of the FJSP. Solvers perform well on small-scale instances, but the problem's complexity grows exponentially. Scaling to data center–sized workloads will require new approximation techniques or faster offline solvers for the carbon-aware FJSP.  
% Our model also simplifies real-world conditions. We do not account for several factors that influence carbon savings, including: Server idle power draw and energy proportionality~\cite{Lefurgy:07, Barroso_warehouse}, limits on task parallelization (i.e., if a task is parallelizable~\cite{fernandez2025hardwarescalingtrendsdiminishing}, and embodied carbon from manufacturing and deployment of servers. \walid{Talk about other approaches to solve this problem.}

\noindent{\textbf{Limitations.}} The main challenge is the complexity of the FJSP. Solvers perform well on small-scale instances, but the problem’s complexity grows exponentially. Scaling to data center–sized workloads will require new approximation techniques or faster offline solvers for the carbon-aware FJSP. Machine learning–based approaches for sustainable systems~\cite{donti2021machine, rolnick2022tackling}, which have shown to accelerate large-scale optimization and stochastic scheduling, may provide a path forward by learning scalable heuristics that approximate optimal solutions.

Our model also simplifies real-world conditions. We do not account for several factors that influence carbon savings, including: Server idle power draw and energy proportionality~\cite{Lefurgy:07, Barroso_warehouse}, limits on task parallelization (i.e., if a task is parallelizable~\cite{fernandez2025hardwarescalingtrendsdiminishing}), and embodied carbon from manufacturing and deployment of servers.

\AL{what insights can we get from solving the problem in an offline manner?}

\AL{time ``bubbles'' in optimal schedule}

\AL{in situations where there are empty time slots even in the optimal makespan schedule -- opportunity to move things around without effecting makespan}

\AL{problem is hard, need online heuristic that can reorder the tasks such that tasks are ``packed'' into low-carbon period -- key motivation for online heuristic}


% \noindent{\textbf{Key insights.}} Prior work~\cite{Hanafy:23:War} showed that scheduling mechanisms often face a trade-off between carbon efficiency, energy efficiency, and performance in homogeneous clusters. We show that heterogeneity intensifies this conflict. Running a workload on the most energy-efficient server may save energy but raise emissions if it lands in a high-carbon period. Running on a faster, less efficient server during a low-carbon period can lower emissions but waste energy.  

% Our offline solver provides \textit{upper bounds on achievable carbon savings}. With $2\times$ the optimal makespan flexibility, a carbon-aware schedule cut emissions by half but tripled energy consumption. This result quantifies the outer limits of what an idealized scheduler could achieve, and helps operators judge whether refining their existing policies is worth the effort.  

% We also quantify the carbon–makespan trade-off: longer makespans open more opportunities to exploit low-carbon windows. Doubling the makespan nearly doubled the savings.  

% Finally, we identify key parameters that shape these bounds. Increasing operations per job from 3 to 5 raised utilization by 20\% and reduced savings by 10\%. Increasing servers from 2 to 5 halved utilization and produced up to $20\times$ higher savings.  

% \noindent{\textbf{Limitations.}} The main challenge is the complexity of the FJSP. Our solver performs well on small-scale instances, but the search space grows exponentially. Scaling to data center–sized workloads will require faster approximation methods or online heuristics with guarantees.  

% Our model also omits factors that affect where and how much savings appear. These include idle power draw~\cite{Lefurgy:07}, lack of energy proportionality~\cite{Barroso_warehouse}, limits on task parallelization~\cite{fernandez2025hardwarescalingtrendsdiminishing}, and embodied carbon from server manufacturing and deployment.  

==> 4-discussion-v3.tex <==
We have shown \textit{upper bounds} on achievable savings in offline settings. and that a trade-off exists between carbon , energy, and makespan. We list our findings for operators to consider when designing online heuristics and select their appropriate trade-off point.

\noindent\textbf{Carbon savings without sacrificing the makespan. } Compared the carbon-agnostic, makespan-minimizer schedule, we can shift the jobs tasks order temporally possibly to low-carbon periods to gain carbon savings. Idle status of the servers enable us to do this. We can utilize the periods when the servers are not utilized in the makespan-minimizer schedule and run the tasks there if they are in low-carbon periods (\autoref{fig:motivation}).

\noindent \textbf{Carbon vs. makespan tradeoff. } Scheduling to only minimize the carbon emissions can increase the makespan. Thus, both metric should be considered when making scheduling decisions. Also, we highlighted the diminishing returns on carbon savings when increasing the makespan (\autoref{fig:main-result}, and allowing $1.5\times$ the optimal makespan seems to be the sweet spot for carbon savings. Introducing more flexibility in scheduling does not yield significant savings.

\noindent \textbf{Carbon vs. energy. } 
Prior work~\cite{Hanafy:23:War} showed that workload scheduling mechanisms often face a trade-off between carbon efficiency, energy efficiency, and performance in homogeneous clusters. Our work reveals that server heterogeneity intensifies this conflict. For instance, running a workload on a faster, less energy-efficient server during a high-carbon period might save energy but will ultimately increase carbon emissions, while using a faster, less efficient server on low-carbon periods may lower emissions but waste energy. 

This trade-off matters for works on heterogeneous environments, such as energy-efficient GPU clusters~\cite{enos2010quantifying, ma2012greengpu}: cluster heterogeneity must be considered if carbon efficiency is also a goal alongside energy efficiency. Operators can tune how much they value carbon versus energy by assigning explicit weights to each.

\noindent{\textbf{Limitations.}} The main challenge is the complexity of the FJSP. Solvers perform well on small-scale instances, but the problem’s complexity grows exponentially. Scaling to data center–sized workloads will require new approximation techniques or faster offline solvers for the carbon-aware FJSP. Machine learning–based approaches for sustainable systems~\cite{donti2021machine, rolnick2022tackling}, which have shown to accelerate large-scale optimization and stochastic scheduling, may provide a path forward by learning scalable heuristics that approximate optimal solutions.

Our model also simplifies real-world conditions. We do not account for several factors that influence carbon savings, including: Server idle power draw and energy proportionality~\cite{Lefurgy:07, Barroso_warehouse}, limits on task parallelization (i.e., if a task is parallelizable~\cite{fernandez2025hardwarescalingtrendsdiminishing}), and embodied carbon from manufacturing and deployment of servers.

==> 4-discussion.tex <==

% {\color{blue}
% outline
% \begin{itemize}
%     \item notable takeaways from the experiments:
%     \begin{itemize}
%         \item carbon savings without increasing makespan
%         \item slightly less carbon savings when servers are heterogeneous (faster machines reduce the optimal makespan, so there is less flexibility in shifting)
%     \end{itemize}
%     % \item discuss about makespan vs. job completion time (done below)
%     % \item challenges
%     % \begin{itemize}
%     %     \item solver complexity -- refer to negative values for carbon savings (outliers) in figure 2 -- relatively small instances and we're already running into these issues -- motivates need for online heuristics
%     % \end{itemize}
% \end{itemize}
% }

% \adaml{going to draft this ``key takeaways'' section today}

A key takeaway of our experiments is that FJSP instances exist where carbon savings can be realized by a carbon-aware solution that \textit{does not} increase makespan (i.e., $S=1$).  This is possible because an optimal carbon-agnostic solution may have idle periods within its schedule, which provides shifting flexibility that can be exploited by a carbon-aware solver to take advantage of low-carbon periods.  Throughout the experiments, changing parameters that shrink the amount and size of idle periods (i.e., increasing server utilization in the optimal solution) correspond to lower carbon savings.  We see this effect, for instance, comparing the results for homogeneous vs. heterogeneous servers (see \autoref{fig:homogen-main} and \autoref{fig:heterogen-main}), or when increasing the number of operations per job (see \autoref{tab:num-ops}).

A key challenge that we run into is the complexity of the FJSP.
Our instances are relatively small and solvers are still reasonably fast, but complexity increases exponentially in the problem size; in order to scale to larger problem sizes (i.e., at the true scale of the motivating application to data center background tasks), further work would be necessary to advance offline approximation techniques for the carbon-aware FJSP problem.

However, even if the complexity issue is addressed, there are additional challenges related to information availability that make a purely offline scheduling technique impractical for the motivating problem.  For instance, our carbon-aware solver knows the time-varying values of carbon intensity, job arrival times, and information about each task's length and energy consumption in advance.  In reality, many/all of these parameters are either completely unknown to the scheduler or must be estimated.  In existing systems, schedulers typically use online algorithms or heuristics to make scheduling decisions ``on-the-fly'' as jobs are submitted.  There are many such techniques with varying complexity, and in many cases, the performance of a given scheduling heuristics depends heavily on the structure of the job type (e.g., genomics vs. ML workloads)~\cite{coleman:25:pisaadversarialapproachcomparing}.

These existing heuristics are primarily designed to optimize performance (i.e., minimize makespan), and do not consider the trade-off between performance and carbon or energy.
Furthermore, even some of these simpler policies (e.g., heterogeneous earliest finish time) still assume knowledge of parameters such as task length, which can be difficult to know in a data center setting~\cite{Kuchnik:2019}.
To compound these challenges, our model of the problem has neglected additional factors such as idle power~\cite{Lefurgy:07}, scaling profiles (i.e., if a task is parallelizable)~\cite{fernandez2025hardwarescalingtrendsdiminishing}, and energy proportionality~\cite{Barroso_warehouse}.

Based on these challenges, there are several fruitful directions to be explored towards the goal of carbon-aware and/or energy-aware flexibility in scheduling for computing workloads with inter-task dependencies.  
For instance, building on the findings of \citet{coleman:25:pisaadversarialapproachcomparing}, one initial task might be to identify specific problem settings where task dependency graphs exhibit some useful structure or patterns that could be exploited by a carbon-aware heuristic.
In designing such a policy, it may be useful to identify existing heuristics that could be repurposed to e.g., elevate carbon emissions or energy usage as a first-class objective.

Critically, a deployed scheduler must often contend with more uncertainty (e.g., about job arrival times, task length, energy usage) than is typically assumed in the theoretical literature on JSP and similar problems.  Addressing this uncertainty while simultaneously dealing with complex trade-offs between carbon and performance calls for novel online policies that can learn and adjust decisions over time using techniques such as feedback-driven optimization or reinforcement learning, embedding context (i.e., current and future carbon intensity, dependency structure) directly into scheduling decisions that hedge against uncertain outcomes.


% {\color{blue}
% Outline for remainder

% - these are the challenges

% - \textbf{what is the next step?}

% - what would be the first problem to solve?  just considering specific structures of precedence? one way to look at DAG structures and approximations  

% - don't hint too much at AL SIGCOMM

% - which approximation techniques are most amenable to tweaks that make them aware of the carbon- and energy-trade-off

% - goal: scheduler that can learn when to be carbon-aware and when to be deadline-aware in an online, feedback-based fashion (using e.g., RL), with potentially limited information about each job as it arrives 

% }

% While our results show that carbon savings can be achieved without impacting \textit{makespan}, we cannot say the same for \textit{average job completion time} (i.e., the time elapsed between a job's submission and its completion).   
%For example, in the \texttt{CAL} grid region, with $n=10$ jobs, $k=3$ operations, and $M=5$ servers, the carbon-aware solver increases average job completion time by $59\%$ in the homogeneous case, and $52\%$ in the heterogeneous case.


% A key challenge that we run into is the complexity of the FJSP.  Solvers are relatively fast for small problems, but since the FJSP is NP-hard, the complexity increases exponentially in the problem size.  We set a uniform solver timeout in our implementation, and this complexity means that for some larger problem sizes (e.g., when the stretch factor, number of jobs, or number of servers increases), our solver cannot find the optimal solution before timing out -- see e.g., \autoref{fig:heterogen-main}, where some outliers for $S > 1$ have negative carbon savings (note that negative savings are intuitively suboptimal since the carbon-agnostic schedule is feasible).  Moreover, the instances that we experiment with (e.g., $10$ jobs, $5$ servers) are relatively small compared to the motivating problem of scheduling real background tasks in data centers.  While one could take advantage of some \textit{approximation} techniques to address the complexity of the problem, we believe this motivates a particular need for \textit{online} algorithms or heuristics for the problem that could simultaneously address the complexity of the problem and the real-world need of scheduling tasks ``on-the-fly'' (i.e., as they are submitted).


==> 5-conclusion.tex <==
% \adaml{conclusions go here}

% \adaml{motivate the need for online algorithms}

Our study of the FJSP demonstrates that exposing inter-task dependencies and machine heterogeneity to a carbon-aware scheduler unlocks sizable carbon gains for batch workloads. Across realistic traces, our experiments show that carbon savings up to 25\% are achievable without affecting makespan. 
%, {\color{blue} outperforming dependency-agnostic schedulers}. 
Solving the FJSP offline for large problem sizes quickly becomes intractable, and real settings in the data center often require scheduling to happen ``on the fly'' and under uncertainty -- this motivates a need for research into novel online policies that incorporate fine-grained knowledge about workloads such as dependencies to fully realize the benefits of carbon-aware shifting.


==> related-work.tex <==
Variants of the job shop scheduling problem (JSP) were first studied in the 1950s to model problems arising in operations research, particularly in machining factories -- see \citet{Xiong:22} for a comprehensive survey.  In a JSP, each job consists of a sequence of operations that must be processed in a specific order on specific machines, with the goal of reducing the overall completion time (makespan).  Job shop scheduling has long been known to be NP-hard~\cite{Garey:76}, so research in the decades since has focused on simple heuristics with performance guarantees (e.g., Graham's list scheduling~\cite{Graham:66}) and approximation techniques with varying degrees of complexity.

One important generalization of the JSP that we leverage in the rest of the paper is the flexible job shop scheduling problem (FJSP) introduced by \citet{Brucker:90}, an extension of job shop in which each operation can be processed on any one of a set of candidate machines rather than a single dedicated machine.  FJSP inherits the combinatorial difficulty of the JSP – it remains NP-hard, as it generalizes the NP-hard job-shop problem and adds another layer of decision-making (the assignment of operations to machines).

While studies in operations research and engineering fields have studied JSP and FJSP in manufacturing contexts, JSP-like problems are also relevant to scheduling problems that arise in computing systems such as scheduling tasks on processors, or scheduling parallel jobs in clusters.  In these settings, jobs (or tasks) often arrive over time and must be scheduled in a real-time (i.e., online) fashion, requiring fast decisions rather than heavy optimization at each step.  Thus, systems often implement fast heuristics such as \textit{earliest task first}~\cite{coleman:25:pisaadversarialapproachcomparing}, with the goal of maximizing throughput (respectively, minimizing makespan).

In recent years, a few studies have considered job shop scheduling problems under competing priorities, such as time-varying costs of production (i.e., time-of-use pricing) and/or total energy usage. For instance, \citet{Park:22} consider a flexible job shop scheduling scenario under time-of-use electricity pricing, aiming to minimize both the makespan and the total energy cost of production.  They solve the problem optimally using solvers and show that it is possible to significantly cut energy costs without compromising productivity in a manufacturing setting.  Several other works consider similar settings~\cite{Terbrack:25, Para:22}, minimizing either energy consumption or energy cost, using a variety of heuristic and approximation methods.  However, most of these works ignore carbon emissions and are almost always grounded in manufacturing or industrial contexts – scheduling physical machines in a factory – rather than scheduling computing jobs in a data center.

Thus, in the rest of the paper, we explore the solution space of schedules for the flexible job shop problem in a setting tailored for computing workloads, using solver tools developed in an operations research context.
By studying the trade-off between carbon and makespan, we show that there are both opportunities and challenges in scheduling tasks with dependencies to reduce their carbon footprint.  In doing so, we hope to illuminate fruitful paths for the development of new schedulers in carbon-aware data centers. 

